Exact logical error rates for magic state cultivation

We compute exactly the acceptance and logical error rates for the distance $d=3$ and $d=5$ magic state cultivation circuits from Clifft [arXiv:2604.27058] and SOFT [arXiv:2512.23037] using Pauli propagation and binary tensor contraction. Actual $T$-gates are studied, not the $S$-gate proxy used for sampling. The calculation includes every fault order at several circuit-level noise strengths ($p$). We provide a series expansion form to the logical error rates, through order $(p/(1-p))^{10}$. The analytical results recover the numerical values from Clifft and SOFT at both $d=3$ and $d=5$ to within their sampling uncertainty. Then, we show that the $d=3$ and $d=5$ circuits actually have fault distances of $d_{\text{fault}}=2$ and $d_{\text{fault}}=3$ respectively, explaining the similar distance degrading effects from the companion code of [Quantum 10, 2134 (2026)].

==> detector_webs/pages.tex <==
\pdfbookmark[1]{d=3, detector 0}{d3_det000}\label{d3_det000}
{\Large $d=3$: detector 0}\qquad{\large $r_{0}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det000.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{0}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{0}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{0}$: M $q_{6}$, line 119.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det000.tikz}}, declared at line 121 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 1}{d3_det001}\label{d3_det001}
{\Large $d=3$: detector 1}\qquad{\large $r_{1}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det001.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{1}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{1}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{1}$: M $q_{14}$, line 119.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det001.tikz}}, declared at line 122 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 2}{d3_det002}\label{d3_det002}
{\Large $d=3$: detector 2}\qquad{\large $r_{2}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det002.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{2}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{2}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{2}$: M $q_{8}$, line 119.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det002.tikz}}, declared at line 123 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 3}{d3_det003}\label{d3_det003}
{\Large $d=3$: detector 3}\qquad{\large $r_{3}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det003.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{3}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{3}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{3}$: M $q_{5}$, line 119.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det003.tikz}}, declared at line 124 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 4}{d3_det004}\label{d3_det004}
{\Large $d=3$: detector 4}\qquad{\large $r_{4}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det004.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{4}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{4}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{4}$: MX $q_{2}$, line 120.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det004.tikz}}, declared at line 125 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 5}{d3_det005}\label{d3_det005}
{\Large $d=3$: detector 5}\qquad{\large $r_{5}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det005.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{5}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{5}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{5}$: MX $q_{11}$, line 120.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det005.tikz}}, declared at line 126 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 6}{d3_det006}\label{d3_det006}
{\Large $d=3$: detector 6}\qquad{\large $r_{6}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det006.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{6}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{6}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{6}$: MX $q_{4}$, line 120.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det006.tikz}}, declared at line 127 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 7}{d3_det007}\label{d3_det007}
{\Large $d=3$: detector 7}\qquad{\large $r_{5}\oplus r_{6}\oplus r_{7}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det007.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{5}+r_{6}+r_{7}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{5}$: MX $q_{11}$, line 120;\quad $r_{6}$: MX $q_{4}$, line 120;\quad $r_{7}$: MX $q_{7}$, line 154.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 62;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{0}$, line 135;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 135;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 135;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 135;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{10}$, line 135;\quad $\ast_{7}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{12}$, line 135;\quad $\ast_{8}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 135.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det007.tikz}}, declared at line 182 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 8}{d3_det008}\label{d3_det008}
{\Large $d=3$: detector 8}\qquad{\large $r_{8}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det008.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{8}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{8}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{8}$: MX $q_{14}$, line 180.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det008.tikz}}, declared at line 183 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 9}{d3_det009}\label{d3_det009}
{\Large $d=3$: detector 9}\qquad{\large $r_{9}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det009.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{9}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{9}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{9}$: MX $q_{11}$, line 180.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det009.tikz}}, declared at line 184 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 10}{d3_det010}\label{d3_det010}
{\Large $d=3$: detector 10}\qquad{\large $r_{7}\oplus r_{10}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det010.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{10}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{7}\oplus r_{10}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 154;\quad $r_{10}$: MX $q_{6}$, line 180.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det010.tikz}}, declared at line 185 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 11}{d3_det011}\label{d3_det011}
{\Large $d=3$: detector 11}\qquad{\large $r_{11}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det011.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{11}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{11}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{11}$: MX $q_{2}$, line 180.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det011.tikz}}, declared at line 186 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 12}{d3_det012}\label{d3_det012}
{\Large $d=3$: detector 12}\qquad{\large $r_{12}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det012.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{12}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{12}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{12}$: MX $q_{8}$, line 180.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det012.tikz}}, declared at line 187 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 13}{d3_det013}\label{d3_det013}
{\Large $d=3$: detector 13}\qquad{\large $r_{13}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det013.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{13}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{13}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{13}$: MX $q_{1}$, line 180.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det013.tikz}}, declared at line 188 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 14}{d3_det014}\label{d3_det014}
{\Large $d=3$: detector 14}\qquad{\large $r_{7}\oplus r_{15}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 16 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det014.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{15}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 154;\quad $r_{15}$: MPP $X_{0}X_{3}X_{7}X_{10}$, line 196.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{0}$, line 135;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 135;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 135;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{10}$, line 135;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{0}$, line 177;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 177;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 177;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{10}$, line 177;\quad $\ast_{9}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{0}$, line 192;\quad $\ast_{10}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 192;\quad $\ast_{11}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 192;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{10}$, line 192;\quad $\ast_{13}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{0}$, line 194;\quad $\ast_{14}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 194;\quad $\ast_{15}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 194;\quad $\ast_{16}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{10}$, line 194.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det014.tikz}}, declared at line 197 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 15}{d3_det015}\label{d3_det015}
{\Large $d=3$: detector 15}\qquad{\large $r_{16}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det015.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{16}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{16}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{16}$: MPP $Z_{0}Z_{3}Z_{7}Z_{10}$, line 196.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det015.tikz}}, declared at line 198 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 16}{d3_det016}\label{d3_det016}
{\Large $d=3$: detector 16}\qquad{\large $r_{7}\oplus r_{17}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 16 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det016.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{17}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 154;\quad $r_{17}$: MPP $X_{3}X_{7}X_{9}X_{12}$, line 196.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 135;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 135;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 135;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{12}$, line 135;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 177;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 177;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{9}$, line 177;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{12}$, line 177;\quad $\ast_{9}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 192;\quad $\ast_{10}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 192;\quad $\ast_{11}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{9}$, line 192;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{12}$, line 192;\quad $\ast_{13}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 194;\quad $\ast_{14}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 194;\quad $\ast_{15}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 194;\quad $\ast_{16}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{12}$, line 194.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det016.tikz}}, declared at line 199 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 17}{d3_det017}\label{d3_det017}
{\Large $d=3$: detector 17}\qquad{\large $r_{18}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det017.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{18}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{18}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{18}$: MPP $Z_{3}Z_{7}Z_{9}Z_{12}$, line 196.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det017.tikz}}, declared at line 200 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 18}{d3_det018}\label{d3_det018}
{\Large $d=3$: detector 18}\qquad{\large $r_{7}\oplus r_{19}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 16 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det018.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{19}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 154;\quad $r_{19}$: MPP $X_{7}X_{10}X_{12}X_{13}$, line 196.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 135;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{10}$, line 135;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{12}$, line 135;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 135;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 177;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{10}$, line 177;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{12}$, line 177;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 177;\quad $\ast_{9}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 192;\quad $\ast_{10}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{10}$, line 192;\quad $\ast_{11}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{12}$, line 192;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 192;\quad $\ast_{13}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 194;\quad $\ast_{14}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{10}$, line 194;\quad $\ast_{15}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{12}$, line 194;\quad $\ast_{16}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 194.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det018.tikz}}, declared at line 201 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=3, detector 19}{d3_det019}\label{d3_det019}
{\Large $d=3$: detector 19}\qquad{\large $r_{20}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d3_det019.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{20}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{20}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{20}$: MPP $Z_{7}Z_{10}Z_{12}Z_{13}$, line 196.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_det019.tikz}}, declared at line 202 of \texttt{\detokenize{data/inputs/clifft_d3_p001.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 0}{d5_det000}\label{d5_det000}
{\Large $d=5$: detector 0}\qquad{\large $r_{0}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det000.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{0}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{0}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{0}$: M $q_{6}$, line 126.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det000.tikz}}, declared at line 128 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 1}{d5_det001}\label{d5_det001}
{\Large $d=5$: detector 1}\qquad{\large $r_{1}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det001.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{1}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{1}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{1}$: M $q_{18}$, line 126.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det001.tikz}}, declared at line 129 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 2}{d5_det002}\label{d5_det002}
{\Large $d=5$: detector 2}\qquad{\large $r_{2}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det002.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{2}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{2}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{2}$: M $q_{8}$, line 126.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det002.tikz}}, declared at line 130 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 3}{d5_det003}\label{d5_det003}
{\Large $d=5$: detector 3}\qquad{\large $r_{3}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det003.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{3}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{3}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{3}$: M $q_{5}$, line 126.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det003.tikz}}, declared at line 131 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 4}{d5_det004}\label{d5_det004}
{\Large $d=5$: detector 4}\qquad{\large $r_{4}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det004.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{4}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{4}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{4}$: MX $q_{2}$, line 127.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det004.tikz}}, declared at line 132 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 5}{d5_det005}\label{d5_det005}
{\Large $d=5$: detector 5}\qquad{\large $r_{5}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det005.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{5}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{5}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{5}$: MX $q_{12}$, line 127.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det005.tikz}}, declared at line 133 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 6}{d5_det006}\label{d5_det006}
{\Large $d=5$: detector 6}\qquad{\large $r_{6}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det006.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{6}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{6}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{6}$: MX $q_{4}$, line 127.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det006.tikz}}, declared at line 134 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 7}{d5_det007}\label{d5_det007}
{\Large $d=5$: detector 7}\qquad{\large $r_{5}\oplus r_{6}\oplus r_{7}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det007.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{5}+r_{6}+r_{7}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{5}$: MX $q_{12}$, line 127;\quad $r_{6}$: MX $q_{4}$, line 127;\quad $r_{7}$: MX $q_{7}$, line 157.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 83;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{0}$, line 143;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 143;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 143;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 143;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{11}$, line 143;\quad $\ast_{7}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 143;\quad $\ast_{8}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{17}$, line 143.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det007.tikz}}, declared at line 177 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 8}{d5_det008}\label{d5_det008}
{\Large $d=5$: detector 8}\qquad{\large $r_{8}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det008.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{8}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{8}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{8}$: MX $q_{18}$, line 176.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det008.tikz}}, declared at line 178 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 9}{d5_det009}\label{d5_det009}
{\Large $d=5$: detector 9}\qquad{\large $r_{9}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det009.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{9}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{9}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{9}$: MX $q_{12}$, line 176.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det009.tikz}}, declared at line 179 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 10}{d5_det010}\label{d5_det010}
{\Large $d=5$: detector 10}\qquad{\large $r_{7}\oplus r_{10}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det010.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{10}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{7}\oplus r_{10}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 157;\quad $r_{10}$: MX $q_{6}$, line 176.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det010.tikz}}, declared at line 180 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 11}{d5_det011}\label{d5_det011}
{\Large $d=5$: detector 11}\qquad{\large $r_{11}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det011.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{11}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{11}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{11}$: MX $q_{2}$, line 176.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det011.tikz}}, declared at line 181 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 12}{d5_det012}\label{d5_det012}
{\Large $d=5$: detector 12}\qquad{\large $r_{12}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det012.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{12}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{12}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{12}$: MX $q_{8}$, line 176.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det012.tikz}}, declared at line 182 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 13}{d5_det013}\label{d5_det013}
{\Large $d=5$: detector 13}\qquad{\large $r_{13}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det013.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{13}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{13}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{13}$: MX $q_{1}$, line 176.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det013.tikz}}, declared at line 183 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 14}{d5_det014}\label{d5_det014}
{\Large $d=5$: detector 14}\qquad{\large $r_{14}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det014.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{14}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{14}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{14}$: M $q_{26}$, line 203.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det014.tikz}}, declared at line 204 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 15}{d5_det015}\label{d5_det015}
{\Large $d=5$: detector 15}\qquad{\large $r_{15}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det015.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{15}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{15}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{15}$: M $q_{33}$, line 203.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det015.tikz}}, declared at line 205 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 16}{d5_det016}\label{d5_det016}
{\Large $d=5$: detector 16}\qquad{\large $r_{16}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det016.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{16}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{16}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{16}$: M $q_{28}$, line 203.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det016.tikz}}, declared at line 206 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 17}{d5_det017}\label{d5_det017}
{\Large $d=5$: detector 17}\qquad{\large $r_{17}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det017.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{17}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{17}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{17}$: M $q_{22}$, line 203.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det017.tikz}}, declared at line 207 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 18}{d5_det018}\label{d5_det018}
{\Large $d=5$: detector 18}\qquad{\large $r_{18}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det018.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{18}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{18}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{18}$: M $q_{16}$, line 203.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det018.tikz}}, declared at line 208 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 19}{d5_det019}\label{d5_det019}
{\Large $d=5$: detector 19}\qquad{\large $r_{7}\oplus r_{36}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det019.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{36}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 157;\quad $r_{36}$: MX $q_{2}$, line 251.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{0}$, line 143;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 143;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 143;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{11}$, line 143;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{0}$, line 174;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 174;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 174;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{11}$, line 174.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det019.tikz}}, declared at line 252 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 20}{d5_det020}\label{d5_det020}
{\Large $d=5$: detector 20}\qquad{\large $r_{7}\oplus r_{35}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det020.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{35}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 157;\quad $r_{35}$: MX $q_{4}$, line 251.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 143;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 143;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 143;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 143;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 174;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 174;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{9}$, line 174;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 174.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det020.tikz}}, declared at line 253 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 21}{d5_det021}\label{d5_det021}
{\Large $d=5$: detector 21}\qquad{\large $r_{27}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det021.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{27}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{27}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{27}$: M $q_{6}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det021.tikz}}, declared at line 254 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 22}{d5_det022}\label{d5_det022}
{\Large $d=5$: detector 22}\qquad{\large $r_{26}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det022.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{26}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{26}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{26}$: M $q_{8}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det022.tikz}}, declared at line 255 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 23}{d5_det023}\label{d5_det023}
{\Large $d=5$: detector 23}\qquad{\large $r_{7}\oplus r_{34}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det023.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{7}+r_{34}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{7}$: MX $q_{7}$, line 157;\quad $r_{34}$: MX $q_{12}$, line 251.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 143;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{11}$, line 143;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 143;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{17}$, line 143;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 174;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{11}$, line 174;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 174;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{17}$, line 174.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det023.tikz}}, declared at line 256 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 24}{d5_det024}\label{d5_det024}
{\Large $d=5$: detector 24}\qquad{\large $r_{32}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det024.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{32}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{32}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{32}$: MX $q_{16}$, line 251.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det024.tikz}}, declared at line 257 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 25}{d5_det025}\label{d5_det025}
{\Large $d=5$: detector 25}\qquad{\large $r_{25}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det025.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{25}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{25}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{25}$: M $q_{18}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det025.tikz}}, declared at line 258 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 26}{d5_det026}\label{d5_det026}
{\Large $d=5$: detector 26}\qquad{\large $r_{23}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det026.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{23}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{23}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{23}$: M $q_{22}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det026.tikz}}, declared at line 259 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 27}{d5_det027}\label{d5_det027}
{\Large $d=5$: detector 27}\qquad{\large $r_{30}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det027.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{30}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{30}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{30}$: MX $q_{26}$, line 251.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det027.tikz}}, declared at line 260 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 28}{d5_det028}\label{d5_det028}
{\Large $d=5$: detector 28}\qquad{\large $r_{29}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det028.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{29}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{29}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{29}$: MX $q_{28}$, line 251.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det028.tikz}}, declared at line 261 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 29}{d5_det029}\label{d5_det029}
{\Large $d=5$: detector 29}\qquad{\large $r_{21}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det029.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{21}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{21}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{21}$: M $q_{33}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det029.tikz}}, declared at line 262 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 30}{d5_det030}\label{d5_det030}
{\Large $d=5$: detector 30}\qquad{\large $r_{20}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det030.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{20}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{20}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{20}$: M $q_{35}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det030.tikz}}, declared at line 263 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 31}{d5_det031}\label{d5_det031}
{\Large $d=5$: detector 31}\qquad{\large $r_{28}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det031.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{28}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{28}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{28}$: MX $q_{37}$, line 251.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det031.tikz}}, declared at line 264 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 32}{d5_det032}\label{d5_det032}
{\Large $d=5$: detector 32}\qquad{\large $r_{19}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det032.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{19}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{19}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{19}$: M $q_{41}$, line 250.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det032.tikz}}, declared at line 265 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 33}{d5_det033}\label{d5_det033}
{\Large $d=5$: detector 33}\qquad{\large $r_{36}\oplus r_{54}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det033.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{36}+r_{54}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{36}\oplus r_{54}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{36}$: MX $q_{2}$, line 251;\quad $r_{54}$: MX $q_{2}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det033.tikz}}, declared at line 311 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 34}{d5_det034}\label{d5_det034}
{\Large $d=5$: detector 34}\qquad{\large $r_{35}\oplus r_{53}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det034.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{35}+r_{53}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{35}\oplus r_{53}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{35}$: MX $q_{4}$, line 251;\quad $r_{53}$: MX $q_{4}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det034.tikz}}, declared at line 312 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 35}{d5_det035}\label{d5_det035}
{\Large $d=5$: detector 35}\qquad{\large $r_{26}\oplus r_{27}\oplus r_{45}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det035.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{26}+r_{27}+r_{45}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{26}\oplus r_{27}\oplus r_{45}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{26}$: M $q_{8}$, line 250;\quad $r_{27}$: M $q_{6}$, line 250;\quad $r_{45}$: M $q_{6}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det035.tikz}}, declared at line 313 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 36}{d5_det036}\label{d5_det036}
{\Large $d=5$: detector 36}\qquad{\large $r_{27}\oplus r_{44}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det036.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{27}+r_{44}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{27}\oplus r_{44}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{27}$: M $q_{6}$, line 250;\quad $r_{44}$: M $q_{8}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det036.tikz}}, declared at line 314 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 37}{d5_det037}\label{d5_det037}
{\Large $d=5$: detector 37}\qquad{\large $r_{34}\oplus r_{52}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det037.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{34}+r_{52}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{34}\oplus r_{52}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{34}$: MX $q_{12}$, line 251;\quad $r_{52}$: MX $q_{12}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det037.tikz}}, declared at line 315 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 38}{d5_det038}\label{d5_det038}
{\Large $d=5$: detector 38}\qquad{\large $r_{51}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det038.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{51}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{51}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{51}$: MX $q_{14}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det038.tikz}}, declared at line 316 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 39}{d5_det039}\label{d5_det039}
{\Large $d=5$: detector 39}\qquad{\large $r_{32}\oplus r_{50}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det039.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{32}+r_{50}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{32}\oplus r_{50}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{32}$: MX $q_{16}$, line 251;\quad $r_{50}$: MX $q_{16}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det039.tikz}}, declared at line 317 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 40}{d5_det040}\label{d5_det040}
{\Large $d=5$: detector 40}\qquad{\large $r_{43}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det040.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{43}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{43}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{43}$: M $q_{18}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det040.tikz}}, declared at line 318 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 41}{d5_det041}\label{d5_det041}
{\Large $d=5$: detector 41}\qquad{\large $r_{42}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det041.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{42}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{42}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{42}$: M $q_{20}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det041.tikz}}, declared at line 319 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 42}{d5_det042}\label{d5_det042}
{\Large $d=5$: detector 42}\qquad{\large $r_{41}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det042.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{41}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{41}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{41}$: M $q_{22}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det042.tikz}}, declared at line 320 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 43}{d5_det043}\label{d5_det043}
{\Large $d=5$: detector 43}\qquad{\large $r_{49}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det043.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{49}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{49}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{49}$: MX $q_{24}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det043.tikz}}, declared at line 321 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 44}{d5_det044}\label{d5_det044}
{\Large $d=5$: detector 44}\qquad{\large $r_{30}\oplus r_{48}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det044.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{30}+r_{48}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{30}\oplus r_{48}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{30}$: MX $q_{26}$, line 251;\quad $r_{48}$: MX $q_{26}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det044.tikz}}, declared at line 322 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 45}{d5_det045}\label{d5_det045}
{\Large $d=5$: detector 45}\qquad{\large $r_{29}\oplus r_{47}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det045.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{29}+r_{47}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{29}\oplus r_{47}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{29}$: MX $q_{28}$, line 251;\quad $r_{47}$: MX $q_{28}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det045.tikz}}, declared at line 323 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 46}{d5_det046}\label{d5_det046}
{\Large $d=5$: detector 46}\qquad{\large $r_{40}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det046.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{40}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{40}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{40}$: M $q_{31}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det046.tikz}}, declared at line 324 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 47}{d5_det047}\label{d5_det047}
{\Large $d=5$: detector 47}\qquad{\large $r_{39}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det047.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{39}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{39}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{39}$: M $q_{33}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det047.tikz}}, declared at line 325 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 48}{d5_det048}\label{d5_det048}
{\Large $d=5$: detector 48}\qquad{\large $r_{21}\oplus r_{38}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det048.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{21}+r_{38}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{21}\oplus r_{38}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{21}$: M $q_{33}$, line 250;\quad $r_{38}$: M $q_{35}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det048.tikz}}, declared at line 326 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 49}{d5_det049}\label{d5_det049}
{\Large $d=5$: detector 49}\qquad{\large $r_{28}\oplus r_{46}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det049.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{28}+r_{46}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{28}\oplus r_{46}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{28}$: MX $q_{37}$, line 251;\quad $r_{46}$: MX $q_{37}$, line 310.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det049.tikz}}, declared at line 327 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 50}{d5_det050}\label{d5_det050}
{\Large $d=5$: detector 50}\qquad{\large $r_{37}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det050.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{37}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{37}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{37}$: M $q_{41}$, line 309.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det050.tikz}}, declared at line 328 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 51}{d5_det051}\label{d5_det051}
{\Large $d=5$: detector 51}\qquad{\large $r_{54}\oplus r_{72}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det051.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{54}+r_{72}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{54}\oplus r_{72}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{54}$: MX $q_{2}$, line 310;\quad $r_{72}$: MX $q_{2}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det051.tikz}}, declared at line 363 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 52}{d5_det052}\label{d5_det052}
{\Large $d=5$: detector 52}\qquad{\large $r_{53}\oplus r_{71}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det052.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{53}+r_{71}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{53}\oplus r_{71}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{53}$: MX $q_{4}$, line 310;\quad $r_{71}$: MX $q_{4}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det052.tikz}}, declared at line 364 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 53}{d5_det053}\label{d5_det053}
{\Large $d=5$: detector 53}\qquad{\large $r_{44}\oplus r_{45}\oplus r_{63}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det053.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{44}+r_{45}+r_{63}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{44}\oplus r_{45}\oplus r_{63}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{44}$: M $q_{8}$, line 309;\quad $r_{45}$: M $q_{6}$, line 309;\quad $r_{63}$: M $q_{6}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det053.tikz}}, declared at line 365 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 54}{d5_det054}\label{d5_det054}
{\Large $d=5$: detector 54}\qquad{\large $r_{45}\oplus r_{62}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det054.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{45}+r_{62}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{45}\oplus r_{62}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{45}$: M $q_{6}$, line 309;\quad $r_{62}$: M $q_{8}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det054.tikz}}, declared at line 366 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 55}{d5_det055}\label{d5_det055}
{\Large $d=5$: detector 55}\qquad{\large $r_{52}\oplus r_{70}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det055.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{52}+r_{70}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{52}\oplus r_{70}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{52}$: MX $q_{12}$, line 310;\quad $r_{70}$: MX $q_{12}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det055.tikz}}, declared at line 367 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 56}{d5_det056}\label{d5_det056}
{\Large $d=5$: detector 56}\qquad{\large $r_{51}\oplus r_{69}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det056.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{51}+r_{69}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{51}\oplus r_{69}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{51}$: MX $q_{14}$, line 310;\quad $r_{69}$: MX $q_{14}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det056.tikz}}, declared at line 368 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 57}{d5_det057}\label{d5_det057}
{\Large $d=5$: detector 57}\qquad{\large $r_{50}\oplus r_{68}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det057.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{50}+r_{68}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{50}\oplus r_{68}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{50}$: MX $q_{16}$, line 310;\quad $r_{68}$: MX $q_{16}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det057.tikz}}, declared at line 369 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 58}{d5_det058}\label{d5_det058}
{\Large $d=5$: detector 58}\qquad{\large $r_{42}\oplus r_{61}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det058.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{42}+r_{61}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{42}\oplus r_{61}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{42}$: M $q_{20}$, line 309;\quad $r_{61}$: M $q_{18}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det058.tikz}}, declared at line 370 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 59}{d5_det059}\label{d5_det059}
{\Large $d=5$: detector 59}\qquad{\large $r_{41}\oplus r_{43}\oplus r_{60}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det059.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{41}+r_{43}+r_{60}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{41}\oplus r_{43}\oplus r_{60}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{41}$: M $q_{22}$, line 309;\quad $r_{43}$: M $q_{18}$, line 309;\quad $r_{60}$: M $q_{20}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det059.tikz}}, declared at line 371 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 60}{d5_det060}\label{d5_det060}
{\Large $d=5$: detector 60}\qquad{\large $r_{42}\oplus r_{59}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det060.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{42}+r_{59}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{42}\oplus r_{59}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{42}$: M $q_{20}$, line 309;\quad $r_{59}$: M $q_{22}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det060.tikz}}, declared at line 372 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 61}{d5_det061}\label{d5_det061}
{\Large $d=5$: detector 61}\qquad{\large $r_{49}\oplus r_{67}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det061.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{49}+r_{67}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{49}\oplus r_{67}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{49}$: MX $q_{24}$, line 310;\quad $r_{67}$: MX $q_{24}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det061.tikz}}, declared at line 373 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 62}{d5_det062}\label{d5_det062}
{\Large $d=5$: detector 62}\qquad{\large $r_{48}\oplus r_{66}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det062.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{48}+r_{66}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{48}\oplus r_{66}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{48}$: MX $q_{26}$, line 310;\quad $r_{66}$: MX $q_{26}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det062.tikz}}, declared at line 374 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 63}{d5_det063}\label{d5_det063}
{\Large $d=5$: detector 63}\qquad{\large $r_{47}\oplus r_{65}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det063.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{47}+r_{65}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{47}\oplus r_{65}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{47}$: MX $q_{28}$, line 310;\quad $r_{65}$: MX $q_{28}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det063.tikz}}, declared at line 375 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 64}{d5_det064}\label{d5_det064}
{\Large $d=5$: detector 64}\qquad{\large $r_{39}\oplus r_{40}\oplus r_{58}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det064.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{39}+r_{40}+r_{58}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{39}\oplus r_{40}\oplus r_{58}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{39}$: M $q_{33}$, line 309;\quad $r_{40}$: M $q_{31}$, line 309;\quad $r_{58}$: M $q_{31}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det064.tikz}}, declared at line 376 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 65}{d5_det065}\label{d5_det065}
{\Large $d=5$: detector 65}\qquad{\large $r_{38}\oplus r_{40}\oplus r_{57}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det065.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{38}+r_{40}+r_{57}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{38}\oplus r_{40}\oplus r_{57}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{38}$: M $q_{35}$, line 309;\quad $r_{40}$: M $q_{31}$, line 309;\quad $r_{57}$: M $q_{33}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det065.tikz}}, declared at line 377 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 66}{d5_det066}\label{d5_det066}
{\Large $d=5$: detector 66}\qquad{\large $r_{39}\oplus r_{56}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det066.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{39}+r_{56}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{39}\oplus r_{56}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{39}$: M $q_{33}$, line 309;\quad $r_{56}$: M $q_{35}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det066.tikz}}, declared at line 378 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 67}{d5_det067}\label{d5_det067}
{\Large $d=5$: detector 67}\qquad{\large $r_{46}\oplus r_{64}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det067.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{46}+r_{64}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{46}\oplus r_{64}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{46}$: MX $q_{37}$, line 310;\quad $r_{64}$: MX $q_{37}$, line 362.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det067.tikz}}, declared at line 379 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 68}{d5_det068}\label{d5_det068}
{\Large $d=5$: detector 68}\qquad{\large $r_{55}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det068.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{55}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{55}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{55}$: M $q_{41}$, line 361.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det068.tikz}}, declared at line 380 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 69}{d5_det069}\label{d5_det069}
{\Large $d=5$: detector 69}\qquad{\large $r_{8}\oplus r_{9}\oplus r_{12}\oplus r_{13}\oplus r_{19}\oplus r_{20}\oplus r_{21}\oplus r_{23}\oplus r_{25}\oplus r_{26}\oplus r_{37}\oplus r_{38}\oplus r_{39}\oplus r_{41}\oplus r_{42}\oplus r_{43}\oplus r_{44}\oplus r_{55}\oplus r_{56}\oplus r_{57}\oplus r_{59}\oplus r_{60}\oplus r_{61}\oplus r_{62}\oplus r_{73}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 26 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det069.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{8}+r_{9}+r_{12}+r_{13}+r_{19}+r_{20}+r_{21}+r_{23}+r_{25}+r_{26}+r_{37}+r_{38}+r_{39}+r_{41}+r_{42}+r_{43}+r_{44}+r_{55}+r_{56}+r_{57}+r_{59}+r_{60}+r_{61}+r_{62}+r_{73}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{8}$: MX $q_{18}$, line 176;\quad $r_{9}$: MX $q_{12}$, line 176;\quad $r_{12}$: MX $q_{8}$, line 176;\quad $r_{13}$: MX $q_{1}$, line 176;\quad $r_{19}$: M $q_{41}$, line 250;\quad $r_{20}$: M $q_{35}$, line 250;\quad $r_{21}$: M $q_{33}$, line 250;\quad $r_{23}$: M $q_{22}$, line 250;\quad $r_{25}$: M $q_{18}$, line 250;\quad $r_{26}$: M $q_{8}$, line 250;\quad $r_{37}$: M $q_{41}$, line 309;\quad $r_{38}$: M $q_{35}$, line 309;\quad $r_{39}$: M $q_{33}$, line 309;\quad $r_{41}$: M $q_{22}$, line 309;\quad $r_{42}$: M $q_{20}$, line 309;\quad $r_{43}$: M $q_{18}$, line 309;\quad $r_{44}$: M $q_{8}$, line 309;\quad $r_{55}$: M $q_{41}$, line 361;\quad $r_{56}$: M $q_{35}$, line 361;\quad $r_{57}$: M $q_{33}$, line 361;\quad $r_{59}$: M $q_{22}$, line 361;\quad $r_{60}$: M $q_{20}$, line 361;\quad $r_{61}$: M $q_{18}$, line 361;\quad $r_{62}$: M $q_{8}$, line 361;\quad $r_{73}$: MX $q_{25}$, line 415.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{0}$, line 174;\quad $\ast_{2}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 174;\quad $\ast_{3}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 174;\quad $\ast_{4}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{9}$, line 174;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{11}$, line 174;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 174;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{17}$, line 174;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{0}$, line 391;\quad $\ast_{9}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 392;\quad $\ast_{10}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 392;\quad $\ast_{11}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 392;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{11}$, line 391;\quad $\ast_{13}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 392;\quad $\ast_{14}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{15}$, line 392;\quad $\ast_{15}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{17}$, line 391;\quad $\ast_{16}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{19}$, line 391;\quad $\ast_{17}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{21}$, line 392;\quad $\ast_{18}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{23}$, line 392;\quad $\ast_{19}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{25}$, line 392;\quad $\ast_{20}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{27}$, line 392;\quad $\ast_{21}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{29}$, line 392;\quad $\ast_{22}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{32}$, line 392;\quad $\ast_{23}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{34}$, line 392;\quad $\ast_{24}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{36}$, line 391;\quad $\ast_{25}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{38}$, line 392;\quad $\ast_{26}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{40}$, line 391.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det069.tikz}}, declared at line 447 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 70}{d5_det070}\label{d5_det070}
{\Large $d=5$: detector 70}\qquad{\large $r_{74}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det070.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{74}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{74}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{74}$: MX $q_{20}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det070.tikz}}, declared at line 448 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 71}{d5_det071}\label{d5_det071}
{\Large $d=5$: detector 71}\qquad{\large $r_{75}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det071.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{75}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{75}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{75}$: MX $q_{22}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det071.tikz}}, declared at line 449 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 72}{d5_det072}\label{d5_det072}
{\Large $d=5$: detector 72}\qquad{\large $r_{76}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det072.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{76}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{76}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{76}$: MX $q_{8}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det072.tikz}}, declared at line 450 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 73}{d5_det073}\label{d5_det073}
{\Large $d=5$: detector 73}\qquad{\large $r_{77}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det073.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{77}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{77}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{77}$: MX $q_{10}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det073.tikz}}, declared at line 451 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 74}{d5_det074}\label{d5_det074}
{\Large $d=5$: detector 74}\qquad{\large $r_{78}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det074.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{78}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{78}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{78}$: MX $q_{2}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det074.tikz}}, declared at line 452 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 75}{d5_det075}\label{d5_det075}
{\Large $d=5$: detector 75}\qquad{\large $r_{79}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det075.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{79}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{79}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{79}$: MX $q_{6}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det075.tikz}}, declared at line 453 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 76}{d5_det076}\label{d5_det076}
{\Large $d=5$: detector 76}\qquad{\large $r_{73}\oplus r_{80}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det076.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{73}+r_{80}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{73}\oplus r_{80}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{73}$: MX $q_{25}$, line 415;\quad $r_{80}$: MX $q_{24}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det076.tikz}}, declared at line 454 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 77}{d5_det077}\label{d5_det077}
{\Large $d=5$: detector 77}\qquad{\large $r_{81}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det077.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{81}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{81}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{81}$: MX $q_{31}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det077.tikz}}, declared at line 455 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 78}{d5_det078}\label{d5_det078}
{\Large $d=5$: detector 78}\qquad{\large $r_{82}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det078.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{82}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{82}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{82}$: MX $q_{39}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det078.tikz}}, declared at line 456 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 79}{d5_det079}\label{d5_det079}
{\Large $d=5$: detector 79}\qquad{\large $r_{83}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det079.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{83}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{83}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{83}$: MX $q_{1}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det079.tikz}}, declared at line 457 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 80}{d5_det080}\label{d5_det080}
{\Large $d=5$: detector 80}\qquad{\large $r_{84}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det080.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{84}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{84}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{84}$: MX $q_{12}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det080.tikz}}, declared at line 458 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 81}{d5_det081}\label{d5_det081}
{\Large $d=5$: detector 81}\qquad{\large $r_{85}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det081.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{85}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{85}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{85}$: MX $q_{18}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det081.tikz}}, declared at line 459 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 82}{d5_det082}\label{d5_det082}
{\Large $d=5$: detector 82}\qquad{\large $r_{86}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det082.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{86}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{86}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{86}$: MX $q_{37}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det082.tikz}}, declared at line 460 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 83}{d5_det083}\label{d5_det083}
{\Large $d=5$: detector 83}\qquad{\large $r_{87}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det083.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{87}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{87}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{87}$: MX $q_{33}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det083.tikz}}, declared at line 461 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 84}{d5_det084}\label{d5_det084}
{\Large $d=5$: detector 84}\qquad{\large $r_{88}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det084.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{88}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{88}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{88}$: MX $q_{14}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det084.tikz}}, declared at line 462 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 85}{d5_det085}\label{d5_det085}
{\Large $d=5$: detector 85}\qquad{\large $r_{89}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det085.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{89}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{89}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{89}$: MX $q_{26}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det085.tikz}}, declared at line 463 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 86}{d5_det086}\label{d5_det086}
{\Large $d=5$: detector 86}\qquad{\large $r_{90}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det086.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{90}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{90}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{90}$: MX $q_{28}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det086.tikz}}, declared at line 464 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 87}{d5_det087}\label{d5_det087}
{\Large $d=5$: detector 87}\qquad{\large $r_{91}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det087.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{91}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{91}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{91}$: MX $q_{30}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det087.tikz}}, declared at line 465 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 88}{d5_det088}\label{d5_det088}
{\Large $d=5$: detector 88}\qquad{\large $r_{92}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det088.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{92}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{92}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{92}$: MX $q_{41}$, line 444.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det088.tikz}}, declared at line 466 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 89}{d5_det089}\label{d5_det089}
{\Large $d=5$: detector 89}\qquad{\large $r_{72}\oplus r_{93}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det089.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{72}+r_{93}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{72}$: MX $q_{2}$, line 362;\quad $r_{93}$: MPP $X_{0}X_{3}X_{7}X_{11}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{0}$, line 391;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 392;\quad $\ast_{4}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{11}$, line 391;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{0}$, line 441;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{11}$, line 441;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 442;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det089.tikz}}, declared at line 472 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 90}{d5_det090}\label{d5_det090}
{\Large $d=5$: detector 90}\qquad{\large $r_{62}\oplus r_{63}\oplus r_{96}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det090.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{62}+r_{63}+r_{96}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{62}\oplus r_{63}\oplus r_{96}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{62}$: M $q_{8}$, line 361;\quad $r_{63}$: M $q_{6}$, line 361;\quad $r_{96}$: MPP $Z_{0}Z_{3}Z_{7}Z_{11}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det090.tikz}}, declared at line 473 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 91}{d5_det091}\label{d5_det091}
{\Large $d=5$: detector 91}\qquad{\large $r_{71}\oplus r_{99}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det091.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{71}+r_{99}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{71}$: MX $q_{4}$, line 362;\quad $r_{99}$: MPP $X_{3}X_{7}X_{9}X_{13}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{3}$, line 392;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 392;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 392;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{3}$, line 442;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 442;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{9}$, line 442;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det091.tikz}}, declared at line 474 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 92}{d5_det092}\label{d5_det092}
{\Large $d=5$: detector 92}\qquad{\large $r_{63}\oplus r_{102}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det092.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{63}+r_{102}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{63}\oplus r_{102}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{63}$: M $q_{6}$, line 361;\quad $r_{102}$: MPP $Z_{3}Z_{7}Z_{9}Z_{13}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det092.tikz}}, declared at line 475 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 93}{d5_det093}\label{d5_det093}
{\Large $d=5$: detector 93}\qquad{\large $r_{70}\oplus r_{73}\oplus r_{105}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 12 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det093.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{70}+r_{73}+r_{105}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{70}$: MX $q_{12}$, line 362;\quad $r_{73}$: MX $q_{25}$, line 415;\quad $r_{105}$: MPP $X_{7}X_{11}X_{13}X_{17}X_{19}X_{25}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{7}$, line 392;\quad $\ast_{2}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{11}$, line 391;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 392;\quad $\ast_{4}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{17}$, line 391;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{19}$, line 391;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{25}$, line 392;\quad $\ast_{7}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{11}$, line 441;\quad $\ast_{8}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{17}$, line 441;\quad $\ast_{9}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{19}$, line 441;\quad $\ast_{10}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{7}$, line 442;\quad $\ast_{11}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 442;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{25}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det093.tikz}}, declared at line 476 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 94}{d5_det094}\label{d5_det094}
{\Large $d=5$: detector 94}\qquad{\large $r_{60}\oplus r_{108}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det094.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{60}+r_{108}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{60}\oplus r_{108}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{60}$: M $q_{20}$, line 361;\quad $r_{108}$: MPP $Z_{7}Z_{11}Z_{13}Z_{17}Z_{19}Z_{25}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det094.tikz}}, declared at line 477 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 95}{d5_det095}\label{d5_det095}
{\Large $d=5$: detector 95}\qquad{\large $r_{69}\oplus r_{94}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 12 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det095.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{69}+r_{94}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{69}$: MX $q_{14}$, line 362;\quad $r_{94}$: MPP $X_{9}X_{13}X_{15}X_{19}X_{21}X_{27}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{9}$, line 392;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{13}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{15}$, line 392;\quad $\ast_{4}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{19}$, line 391;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{21}$, line 392;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{27}$, line 392;\quad $\ast_{7}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{19}$, line 441;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{9}$, line 442;\quad $\ast_{9}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{13}$, line 442;\quad $\ast_{10}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{15}$, line 442;\quad $\ast_{11}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{21}$, line 442;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{27}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det095.tikz}}, declared at line 478 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 96}{d5_det096}\label{d5_det096}
{\Large $d=5$: detector 96}\qquad{\large $r_{59}\oplus r_{61}\oplus r_{97}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det096.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{59}+r_{61}+r_{97}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{59}\oplus r_{61}\oplus r_{97}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{59}$: M $q_{22}$, line 361;\quad $r_{61}$: M $q_{18}$, line 361;\quad $r_{97}$: MPP $Z_{9}Z_{13}Z_{15}Z_{19}Z_{21}Z_{27}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det096.tikz}}, declared at line 479 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 97}{d5_det097}\label{d5_det097}
{\Large $d=5$: detector 97}\qquad{\large $r_{68}\oplus r_{100}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det097.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{68}+r_{100}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{68}$: MX $q_{16}$, line 362;\quad $r_{100}$: MPP $X_{15}X_{21}X_{23}X_{29}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{15}$, line 392;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{21}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{23}$, line 392;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{29}$, line 392;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{15}$, line 442;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{21}$, line 442;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{23}$, line 442;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{29}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det097.tikz}}, declared at line 480 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 98}{d5_det098}\label{d5_det098}
{\Large $d=5$: detector 98}\qquad{\large $r_{60}\oplus r_{103}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det098.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{60}+r_{103}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{60}\oplus r_{103}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{60}$: M $q_{20}$, line 361;\quad $r_{103}$: MPP $Z_{15}Z_{21}Z_{23}Z_{29}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det098.tikz}}, declared at line 481 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 99}{d5_det099}\label{d5_det099}
{\Large $d=5$: detector 99}\qquad{\large $r_{67}\oplus r_{73}\oplus r_{95}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det099.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{67}+r_{73}+r_{95}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{67}$: MX $q_{24}$, line 362;\quad $r_{73}$: MX $q_{25}$, line 415;\quad $r_{95}$: MPP $X_{17}X_{25}X_{32}X_{36}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{17}$, line 391;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{25}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{32}$, line 392;\quad $\ast_{4}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{36}$, line 391;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{17}$, line 441;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{36}$, line 441;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{25}$, line 442;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{32}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det099.tikz}}, declared at line 482 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 100}{d5_det100}\label{d5_det100}
{\Large $d=5$: detector 100}\qquad{\large $r_{57}\oplus r_{58}\oplus r_{98}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det100.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{57}+r_{58}+r_{98}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{57}\oplus r_{58}\oplus r_{98}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{57}$: M $q_{33}$, line 361;\quad $r_{58}$: M $q_{31}$, line 361;\quad $r_{98}$: MPP $Z_{17}Z_{25}Z_{32}Z_{36}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det100.tikz}}, declared at line 483 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 101}{d5_det101}\label{d5_det101}
{\Large $d=5$: detector 101}\qquad{\large $r_{66}\oplus r_{73}\oplus r_{101}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 12 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det101.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{66}+r_{73}+r_{101}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{66}$: MX $q_{26}$, line 362;\quad $r_{73}$: MX $q_{25}$, line 415;\quad $r_{101}$: MPP $X_{19}X_{25}X_{27}X_{32}X_{34}X_{38}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{19}$, line 391;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{25}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{27}$, line 392;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{32}$, line 392;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{34}$, line 392;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{38}$, line 392;\quad $\ast_{7}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{19}$, line 441;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{25}$, line 442;\quad $\ast_{9}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{27}$, line 442;\quad $\ast_{10}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{32}$, line 442;\quad $\ast_{11}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{34}$, line 442;\quad $\ast_{12}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{38}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det101.tikz}}, declared at line 484 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 102}{d5_det102}\label{d5_det102}
{\Large $d=5$: detector 102}\qquad{\large $r_{56}\oplus r_{58}\oplus r_{104}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det102.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{56}+r_{58}+r_{104}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{56}\oplus r_{58}\oplus r_{104}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{56}$: M $q_{35}$, line 361;\quad $r_{58}$: M $q_{31}$, line 361;\quad $r_{104}$: MPP $Z_{19}Z_{25}Z_{27}Z_{32}Z_{34}Z_{38}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det102.tikz}}, declared at line 485 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 103}{d5_det103}\label{d5_det103}
{\Large $d=5$: detector 103}\qquad{\large $r_{65}\oplus r_{106}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det103.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{65}+r_{106}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{65}$: MX $q_{28}$, line 362;\quad $r_{106}$: MPP $X_{21}X_{27}X_{29}X_{34}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{21}$, line 392;\quad $\ast_{2}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{27}$, line 392;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{29}$, line 392;\quad $\ast_{4}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{34}$, line 392;\quad $\ast_{5}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{21}$, line 442;\quad $\ast_{6}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{27}$, line 442;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{29}$, line 442;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{34}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det103.tikz}}, declared at line 486 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 104}{d5_det104}\label{d5_det104}
{\Large $d=5$: detector 104}\qquad{\large $r_{57}\oplus r_{109}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det104.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{57}+r_{109}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{57}\oplus r_{109}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{57}$: M $q_{33}$, line 361;\quad $r_{109}$: MPP $Z_{21}Z_{27}Z_{29}Z_{34}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det104.tikz}}, declared at line 487 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 105}{d5_det105}\label{d5_det105}
{\Large $d=5$: detector 105}\qquad{\large $r_{64}\oplus r_{107}=0$}\par
\textbf{Phase-dependent.} Closed semiweb with 8 defects, every one at a $T$ or $T^\dagger$ spider. No closed Pauli web without defects has these records. With every $T$ replaced by $S$ (the $S$ proxy), the same labels are a Pauli web.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det105.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r,\boldsymbol\delta}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{64}+r_{107}}$. \qquad $D_{\boldsymbol r,\boldsymbol\delta}$ has the marked phases changed, so this identity alone does not fix the parity.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{64}$: MX $q_{37}$, line 362;\quad $r_{107}$: MPP $X_{32}X_{36}X_{38}X_{40}$, line 470.\end{minipage}
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\ast_{1}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{32}$, line 392;\quad $\ast_{2}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{36}$, line 391;\quad $\ast_{3}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{38}$, line 392;\quad $\ast_{4}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{40}$, line 391;\quad $\ast_{5}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{36}$, line 441;\quad $\ast_{6}$: $\delta=-\frac{\pi}{2}$ at $T^\dagger$ on $q_{40}$, line 441;\quad $\ast_{7}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{32}$, line 442;\quad $\ast_{8}$: $\delta=\frac{\pi}{2}$ at $T$ on $q_{38}$, line 442.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det105.tikz}}, declared at line 488 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage

\pdfbookmark[1]{d=5, detector 106}{d5_det106}\label{d5_det106}
{\Large $d=5$: detector 106}\qquad{\large $r_{110}=0$}\par
\textbf{Phase-independent.} Closed Pauli web with no defects, so the check holds for any angle at every $T$ spider.
\begin{center}
\semiwebinput{detector_webs/diagrams/d5_det106.tikz}
\end{center}
\vspace{-1mm}
$D_{\boldsymbol r}=\lambda(\boldsymbol r)\,D_{\boldsymbol r}$, \quad $\lambda(\boldsymbol r)=(-1)^{r_{110}}$. \qquad So $D_{\boldsymbol r}=0$ unless $r_{110}=0$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Records: $r_{110}$: MPP $Z_{32}Z_{36}Z_{38}Z_{40}$, line 470.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_det106.tikz}}, declared at line 489 of \texttt{\detokenize{data/inputs/soft_cultivation_d5_p0005.stim}}}
\newpage


==> semiwebs/pages.tex <==
\pdfbookmark[1]{d=3: Incoming Paulis}{group-3-incoming}
\pdfbookmark[2]{d=3, element 1: Incoming Paulis}{d3_001}
{\Large $d=3$: incoming $X_{0}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_001.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{0}$, \quad $P_{\rm out}=X_{0}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_001.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 2: Incoming Paulis}{d3_002}
{\Large $d=3$: incoming $Z_{0}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_002.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{0}$, \quad $P_{\rm out}=Z_{0}Z_{7}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_002.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 3: Incoming Paulis}{d3_003}
{\Large $d=3$: incoming $X_{3}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_003.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{3}$, \quad $P_{\rm out}=X_{3}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_003.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 4: Incoming Paulis}{d3_004}
{\Large $d=3$: incoming $Z_{3}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_004.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{3}$, \quad $P_{\rm out}=Z_{3}Z_{7}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_004.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 5: Incoming Paulis}{d3_005}
{\Large $d=3$: incoming $X_{7}$}\par
Incoming Paulis. 7 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_005.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{7}$, \quad $P_{\rm out}=X_{0}X_{3}X_{9}X_{10}X_{12}X_{13}$, \quad $\lambda=e^{i\frac{5\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$;\quad $\delta_{3}=-\frac{\pi}{2}$;\quad $\delta_{4}=-\frac{\pi}{2}$;\quad $\delta_{5}=-\frac{\pi}{2}$;\quad $\delta_{6}=-\frac{\pi}{2}$;\quad $\delta_{7}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_005.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 6: Incoming Paulis}{d3_006}
{\Large $d=3$: incoming $Z_{7}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_006.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{7}$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_006.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 7: Incoming Paulis}{d3_007}
{\Large $d=3$: incoming $X_{9}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_007.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{9}$, \quad $P_{\rm out}=X_{9}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_007.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 8: Incoming Paulis}{d3_008}
{\Large $d=3$: incoming $Z_{9}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_008.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{9}$, \quad $P_{\rm out}=Z_{7}Z_{9}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_008.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 9: Incoming Paulis}{d3_009}
{\Large $d=3$: incoming $X_{10}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_009.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{10}$, \quad $P_{\rm out}=X_{10}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_009.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 10: Incoming Paulis}{d3_010}
{\Large $d=3$: incoming $Z_{10}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_010.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{10}$, \quad $P_{\rm out}=Z_{7}Z_{10}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_010.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 11: Incoming Paulis}{d3_011}
{\Large $d=3$: incoming $X_{12}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_011.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{12}$, \quad $P_{\rm out}=X_{12}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_011.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 12: Incoming Paulis}{d3_012}
{\Large $d=3$: incoming $Z_{12}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_012.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{12}$, \quad $P_{\rm out}=Z_{7}Z_{12}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_012.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 13: Incoming Paulis}{d3_013}
{\Large $d=3$: incoming $X_{13}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_013.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{13}$, \quad $P_{\rm out}=X_{13}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_013.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 14: Incoming Paulis}{d3_014}
{\Large $d=3$: incoming $Z_{13}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_014.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{13}$, \quad $P_{\rm out}=Z_{7}Z_{13}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_014.tikz}}}
\newpage
\pdfbookmark[1]{d=3: Additional output support}{group-3-output}
\pdfbookmark[2]{d=3, element 15: Additional output support}{d3_015}
{\Large $d=3$: basis element 15}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_015.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{0}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_015.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 16: Additional output support}{d3_016}
{\Large $d=3$: basis element 16}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_016.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{3}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_016.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 17: Additional output support}{d3_017}
{\Large $d=3$: basis element 17}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_017.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{7}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_017.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 18: Additional output support}{d3_018}
{\Large $d=3$: basis element 18}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_018.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{9}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_018.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 19: Additional output support}{d3_019}
{\Large $d=3$: basis element 19}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_019.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{10}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_019.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 20: Additional output support}{d3_020}
{\Large $d=3$: basis element 20}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_020.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{12}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_020.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 21: Additional output support}{d3_021}
{\Large $d=3$: basis element 21}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_021.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{13}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_021.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 22: Additional output support}{d3_022}
{\Large $d=3$: basis element 22}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_022.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{0}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_022.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 23: Additional output support}{d3_023}
{\Large $d=3$: basis element 23}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_023.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{3}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_023.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 24: Additional output support}{d3_024}
{\Large $d=3$: basis element 24}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_024.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{7}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_024.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 25: Additional output support}{d3_025}
{\Large $d=3$: basis element 25}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_025.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{9}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_025.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 26: Additional output support}{d3_026}
{\Large $d=3$: basis element 26}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_026.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{10}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_026.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 27: Additional output support}{d3_027}
{\Large $d=3$: basis element 27}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_027.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{12}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_027.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 28: Additional output support}{d3_028}
{\Large $d=3$: basis element 28}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_028.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{13}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_028.tikz}}}
\newpage
\pdfbookmark[1]{d=3: No boundary support}{group-3-internal}
\pdfbookmark[2]{d=3, element 29: No boundary support}{d3_029}
{\Large $d=3$: basis element 29}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_029.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d3_029.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 30: No boundary support}{d3_030}
{\Large $d=3$: basis element 30}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_030.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d3_030.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 31: No boundary support}{d3_031}
{\Large $d=3$: basis element 31}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_031.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d3_031.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 32: No boundary support}{d3_032}
{\Large $d=3$: basis element 32}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_032.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d3_032.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 33: No boundary support}{d3_033}
{\Large $d=3$: basis element 33}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_033.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d3_033.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 34: No boundary support}{d3_034}
{\Large $d=3$: basis element 34}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_034.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d3_034.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 35: No boundary support}{d3_035}
{\Large $d=3$: basis element 35}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_035.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_035.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 36: No boundary support}{d3_036}
{\Large $d=3$: basis element 36}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_036.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_036.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 37: No boundary support}{d3_037}
{\Large $d=3$: basis element 37}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_037.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_037.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 38: No boundary support}{d3_038}
{\Large $d=3$: basis element 38}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_038.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_038.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 39: No boundary support}{d3_039}
{\Large $d=3$: basis element 39}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_039.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_039.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 40: No boundary support}{d3_040}
{\Large $d=3$: basis element 40}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_040.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_040.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 41: No boundary support}{d3_041}
{\Large $d=3$: basis element 41}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_041.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_041.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 42: No boundary support}{d3_042}
{\Large $d=3$: basis element 42}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_042.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_042.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 43: No boundary support}{d3_043}
{\Large $d=3$: basis element 43}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_043.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_043.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 44: No boundary support}{d3_044}
{\Large $d=3$: basis element 44}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_044.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_044.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 45: No boundary support}{d3_045}
{\Large $d=3$: basis element 45}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_045.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_045.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 46: No boundary support}{d3_046}
{\Large $d=3$: basis element 46}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_046.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_046.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 47: No boundary support}{d3_047}
{\Large $d=3$: basis element 47}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_047.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_047.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 48: No boundary support}{d3_048}
{\Large $d=3$: basis element 48}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_048.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_048.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 49: No boundary support}{d3_049}
{\Large $d=3$: basis element 49}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_049.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_049.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 50: No boundary support}{d3_050}
{\Large $d=3$: basis element 50}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_050.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_050.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 51: No boundary support}{d3_051}
{\Large $d=3$: basis element 51}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_051.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_051.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 52: No boundary support}{d3_052}
{\Large $d=3$: basis element 52}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_052.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_052.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 53: No boundary support}{d3_053}
{\Large $d=3$: basis element 53}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_053.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_053.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 54: No boundary support}{d3_054}
{\Large $d=3$: basis element 54}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_054.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_054.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 55: No boundary support}{d3_055}
{\Large $d=3$: basis element 55}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_055.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_055.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 56: No boundary support}{d3_056}
{\Large $d=3$: basis element 56}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_056.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_056.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 57: No boundary support}{d3_057}
{\Large $d=3$: basis element 57}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_057.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_057.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 58: No boundary support}{d3_058}
{\Large $d=3$: basis element 58}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_058.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_058.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 59: No boundary support}{d3_059}
{\Large $d=3$: basis element 59}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_059.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_059.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 60: No boundary support}{d3_060}
{\Large $d=3$: basis element 60}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_060.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_060.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 61: No boundary support}{d3_061}
{\Large $d=3$: basis element 61}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_061.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_061.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 62: No boundary support}{d3_062}
{\Large $d=3$: basis element 62}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_062.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_062.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 63: No boundary support}{d3_063}
{\Large $d=3$: basis element 63}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_063.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_063.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 64: No boundary support}{d3_064}
{\Large $d=3$: basis element 64}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_064.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_064.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 65: No boundary support}{d3_065}
{\Large $d=3$: basis element 65}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_065.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_065.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 66: No boundary support}{d3_066}
{\Large $d=3$: basis element 66}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_066.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_066.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 67: No boundary support}{d3_067}
{\Large $d=3$: basis element 67}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_067.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_067.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 68: No boundary support}{d3_068}
{\Large $d=3$: basis element 68}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_068.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_068.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 69: No boundary support}{d3_069}
{\Large $d=3$: basis element 69}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_069.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_069.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 70: No boundary support}{d3_070}
{\Large $d=3$: basis element 70}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_070.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_070.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 71: No boundary support}{d3_071}
{\Large $d=3$: basis element 71}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_071.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_071.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 72: No boundary support}{d3_072}
{\Large $d=3$: basis element 72}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_072.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_072.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 73: No boundary support}{d3_073}
{\Large $d=3$: basis element 73}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_073.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_073.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 74: No boundary support}{d3_074}
{\Large $d=3$: basis element 74}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_074.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_074.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 75: No boundary support}{d3_075}
{\Large $d=3$: basis element 75}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_075.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_075.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 76: No boundary support}{d3_076}
{\Large $d=3$: basis element 76}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_076.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_076.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 77: No boundary support}{d3_077}
{\Large $d=3$: basis element 77}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_077.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_077.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 78: No boundary support}{d3_078}
{\Large $d=3$: basis element 78}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_078.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_078.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 79: No boundary support}{d3_079}
{\Large $d=3$: basis element 79}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_079.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_079.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 80: No boundary support}{d3_080}
{\Large $d=3$: basis element 80}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_080.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_080.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 81: No boundary support}{d3_081}
{\Large $d=3$: basis element 81}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_081.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_081.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 82: No boundary support}{d3_082}
{\Large $d=3$: basis element 82}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_082.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_082.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 83: No boundary support}{d3_083}
{\Large $d=3$: basis element 83}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_083.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_083.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 84: No boundary support}{d3_084}
{\Large $d=3$: basis element 84}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_084.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_084.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 85: No boundary support}{d3_085}
{\Large $d=3$: basis element 85}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_085.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_085.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 86: No boundary support}{d3_086}
{\Large $d=3$: basis element 86}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_086.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_086.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 87: No boundary support}{d3_087}
{\Large $d=3$: basis element 87}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_087.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_087.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 88: No boundary support}{d3_088}
{\Large $d=3$: basis element 88}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_088.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_088.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 89: No boundary support}{d3_089}
{\Large $d=3$: basis element 89}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_089.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_089.tikz}}}
\newpage
\pdfbookmark[2]{d=3, element 90: No boundary support}{d3_090}
{\Large $d=3$: basis element 90}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d3_090.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d3_090.tikz}}}
\newpage
\pdfbookmark[1]{d=5: Incoming Paulis}{group-5-incoming}
\pdfbookmark[2]{d=5, element 1: Incoming Paulis}{d5_001}
{\Large $d=5$: incoming $X_{0}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_001.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{0}$, \quad $P_{\rm out}=X_{0}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=-\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_001.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 2: Incoming Paulis}{d5_002}
{\Large $d=5$: incoming $Z_{0}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_002.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{0}$, \quad $P_{\rm out}=Z_{0}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_002.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 3: Incoming Paulis}{d5_003}
{\Large $d=5$: incoming $X_{3}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_003.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{3}$, \quad $P_{\rm out}=X_{3}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_003.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 4: Incoming Paulis}{d5_004}
{\Large $d=5$: incoming $Z_{3}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_004.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{3}$, \quad $P_{\rm out}=Z_{3}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_004.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 5: Incoming Paulis}{d5_005}
{\Large $d=5$: incoming $X_{7}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_005.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{7}$, \quad $P_{\rm out}=X_{7}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_005.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 6: Incoming Paulis}{d5_006}
{\Large $d=5$: incoming $Z_{7}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_006.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{7}$, \quad $P_{\rm out}=Z_{7}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_006.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 7: Incoming Paulis}{d5_007}
{\Large $d=5$: incoming $X_{9}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_007.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{9}$, \quad $P_{\rm out}=X_{9}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_007.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 8: Incoming Paulis}{d5_008}
{\Large $d=5$: incoming $Z_{9}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_008.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{9}$, \quad $P_{\rm out}=Z_{9}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_008.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 9: Incoming Paulis}{d5_009}
{\Large $d=5$: incoming $X_{11}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_009.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{11}$, \quad $P_{\rm out}=X_{11}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=-\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_009.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 10: Incoming Paulis}{d5_010}
{\Large $d=5$: incoming $Z_{11}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_010.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{11}$, \quad $P_{\rm out}=Z_{11}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_010.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 11: Incoming Paulis}{d5_011}
{\Large $d=5$: incoming $X_{13}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_011.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{13}$, \quad $P_{\rm out}=X_{13}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_011.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 12: Incoming Paulis}{d5_012}
{\Large $d=5$: incoming $Z_{13}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_012.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{13}$, \quad $P_{\rm out}=Z_{13}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_012.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 13: Incoming Paulis}{d5_013}
{\Large $d=5$: incoming $X_{15}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_013.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{15}$, \quad $P_{\rm out}=X_{15}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_013.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 14: Incoming Paulis}{d5_014}
{\Large $d=5$: incoming $Z_{15}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_014.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{15}$, \quad $P_{\rm out}=Z_{15}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_014.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 15: Incoming Paulis}{d5_015}
{\Large $d=5$: incoming $X_{17}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_015.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{17}$, \quad $P_{\rm out}=X_{17}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=-\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_015.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 16: Incoming Paulis}{d5_016}
{\Large $d=5$: incoming $Z_{17}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_016.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{17}$, \quad $P_{\rm out}=Z_{17}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_016.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 17: Incoming Paulis}{d5_017}
{\Large $d=5$: incoming $X_{19}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_017.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{19}$, \quad $P_{\rm out}=X_{19}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=-\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_017.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 18: Incoming Paulis}{d5_018}
{\Large $d=5$: incoming $Z_{19}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_018.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{19}$, \quad $P_{\rm out}=Z_{19}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_018.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 19: Incoming Paulis}{d5_019}
{\Large $d=5$: incoming $X_{21}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_019.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{21}$, \quad $P_{\rm out}=X_{21}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_019.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 20: Incoming Paulis}{d5_020}
{\Large $d=5$: incoming $Z_{21}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_020.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{21}$, \quad $P_{\rm out}=Z_{21}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_020.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 21: Incoming Paulis}{d5_021}
{\Large $d=5$: incoming $X_{23}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_021.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{23}$, \quad $P_{\rm out}=X_{23}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_021.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 22: Incoming Paulis}{d5_022}
{\Large $d=5$: incoming $Z_{23}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_022.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{23}$, \quad $P_{\rm out}=Z_{23}Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_022.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 23: Incoming Paulis}{d5_023}
{\Large $d=5$: incoming $X_{25}$}\par
Incoming Paulis. 19 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_023.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{25}$, \quad $P_{\rm out}=X_{0}X_{3}X_{7}X_{9}X_{11}X_{13}X_{15}X_{17}X_{19}X_{21}X_{23}X_{27}X_{29}X_{32}X_{34}X_{36}X_{38}X_{40}$, \quad $\lambda=e^{i\frac{5\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$;\quad $\delta_{3}=-\frac{\pi}{2}$;\quad $\delta_{4}=-\frac{\pi}{2}$;\quad $\delta_{5}=-\frac{\pi}{2}$;\quad $\delta_{6}=\frac{\pi}{2}$;\quad $\delta_{7}=-\frac{\pi}{2}$;\quad $\delta_{8}=-\frac{\pi}{2}$;\quad $\delta_{9}=\frac{\pi}{2}$;\quad $\delta_{10}=\frac{\pi}{2}$;\quad $\delta_{11}=-\frac{\pi}{2}$;\quad $\delta_{12}=-\frac{\pi}{2}$;\quad $\delta_{13}=-\frac{\pi}{2}$;\quad $\delta_{14}=-\frac{\pi}{2}$;\quad $\delta_{15}=-\frac{\pi}{2}$;\quad $\delta_{16}=-\frac{\pi}{2}$;\quad $\delta_{17}=\frac{\pi}{2}$;\quad $\delta_{18}=-\frac{\pi}{2}$;\quad $\delta_{19}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_023.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 24: Incoming Paulis}{d5_024}
{\Large $d=5$: incoming $Z_{25}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_024.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{25}$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_024.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 25: Incoming Paulis}{d5_025}
{\Large $d=5$: incoming $X_{27}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_025.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{27}$, \quad $P_{\rm out}=X_{27}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_025.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 26: Incoming Paulis}{d5_026}
{\Large $d=5$: incoming $Z_{27}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_026.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{27}$, \quad $P_{\rm out}=Z_{25}Z_{27}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_026.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 27: Incoming Paulis}{d5_027}
{\Large $d=5$: incoming $X_{29}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_027.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{29}$, \quad $P_{\rm out}=X_{29}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_027.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 28: Incoming Paulis}{d5_028}
{\Large $d=5$: incoming $Z_{29}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_028.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{29}$, \quad $P_{\rm out}=Z_{25}Z_{29}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_028.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 29: Incoming Paulis}{d5_029}
{\Large $d=5$: incoming $X_{32}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_029.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{32}$, \quad $P_{\rm out}=X_{32}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_029.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 30: Incoming Paulis}{d5_030}
{\Large $d=5$: incoming $Z_{32}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_030.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{32}$, \quad $P_{\rm out}=Z_{25}Z_{32}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_030.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 31: Incoming Paulis}{d5_031}
{\Large $d=5$: incoming $X_{34}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_031.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{34}$, \quad $P_{\rm out}=X_{34}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_031.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 32: Incoming Paulis}{d5_032}
{\Large $d=5$: incoming $Z_{34}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_032.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{34}$, \quad $P_{\rm out}=Z_{25}Z_{34}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_032.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 33: Incoming Paulis}{d5_033}
{\Large $d=5$: incoming $X_{36}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_033.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{36}$, \quad $P_{\rm out}=X_{36}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=-\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_033.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 34: Incoming Paulis}{d5_034}
{\Large $d=5$: incoming $Z_{36}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_034.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{36}$, \quad $P_{\rm out}=Z_{25}Z_{36}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_034.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 35: Incoming Paulis}{d5_035}
{\Large $d=5$: incoming $X_{38}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_035.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{38}$, \quad $P_{\rm out}=X_{38}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\frac{\pi}{2}$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_035.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 36: Incoming Paulis}{d5_036}
{\Large $d=5$: incoming $Z_{38}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_036.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{38}$, \quad $P_{\rm out}=Z_{25}Z_{38}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_036.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 37: Incoming Paulis}{d5_037}
{\Large $d=5$: incoming $X_{40}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_037.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=X_{40}$, \quad $P_{\rm out}=X_{40}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=-\frac{\pi}{2}$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_037.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 38: Incoming Paulis}{d5_038}
{\Large $d=5$: incoming $Z_{40}$}\par
Incoming Paulis. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_038.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=Z_{40}$, \quad $P_{\rm out}=Z_{25}Z_{40}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_038.tikz}}}
\newpage
\pdfbookmark[1]{d=5: Additional output support}{group-5-output}
\pdfbookmark[2]{d=5, element 39: Additional output support}{d5_039}
{\Large $d=5$: basis element 39}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_039.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{0}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_039.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 40: Additional output support}{d5_040}
{\Large $d=5$: basis element 40}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_040.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{3}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_040.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 41: Additional output support}{d5_041}
{\Large $d=5$: basis element 41}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_041.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{7}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_041.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 42: Additional output support}{d5_042}
{\Large $d=5$: basis element 42}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_042.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{9}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_042.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 43: Additional output support}{d5_043}
{\Large $d=5$: basis element 43}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_043.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{11}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_043.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 44: Additional output support}{d5_044}
{\Large $d=5$: basis element 44}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_044.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{13}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_044.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 45: Additional output support}{d5_045}
{\Large $d=5$: basis element 45}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_045.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{15}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_045.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 46: Additional output support}{d5_046}
{\Large $d=5$: basis element 46}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_046.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{17}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_046.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 47: Additional output support}{d5_047}
{\Large $d=5$: basis element 47}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_047.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{19}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_047.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 48: Additional output support}{d5_048}
{\Large $d=5$: basis element 48}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_048.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{21}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_048.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 49: Additional output support}{d5_049}
{\Large $d=5$: basis element 49}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_049.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{23}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_049.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 50: Additional output support}{d5_050}
{\Large $d=5$: basis element 50}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_050.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{25}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_050.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 51: Additional output support}{d5_051}
{\Large $d=5$: basis element 51}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_051.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{27}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_051.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 52: Additional output support}{d5_052}
{\Large $d=5$: basis element 52}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_052.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{29}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_052.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 53: Additional output support}{d5_053}
{\Large $d=5$: basis element 53}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_053.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{32}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_053.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 54: Additional output support}{d5_054}
{\Large $d=5$: basis element 54}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_054.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{34}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_054.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 55: Additional output support}{d5_055}
{\Large $d=5$: basis element 55}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_055.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{36}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_055.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 56: Additional output support}{d5_056}
{\Large $d=5$: basis element 56}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_056.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{38}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_056.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 57: Additional output support}{d5_057}
{\Large $d=5$: basis element 57}\par
Additional output support. 1 phase defect.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_057.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=Z_{40}$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_057.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 58: Additional output support}{d5_058}
{\Large $d=5$: basis element 58}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_058.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{0}$, \quad $\lambda=e^{i\frac{7\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_058.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 59: Additional output support}{d5_059}
{\Large $d=5$: basis element 59}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_059.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{3}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_059.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 60: Additional output support}{d5_060}
{\Large $d=5$: basis element 60}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_060.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{7}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_060.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 61: Additional output support}{d5_061}
{\Large $d=5$: basis element 61}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_061.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{9}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_061.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 62: Additional output support}{d5_062}
{\Large $d=5$: basis element 62}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_062.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{11}$, \quad $\lambda=e^{i\frac{7\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_062.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 63: Additional output support}{d5_063}
{\Large $d=5$: basis element 63}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_063.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{13}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_063.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 64: Additional output support}{d5_064}
{\Large $d=5$: basis element 64}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_064.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{15}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_064.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 65: Additional output support}{d5_065}
{\Large $d=5$: basis element 65}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_065.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{17}$, \quad $\lambda=e^{i\frac{7\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_065.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 66: Additional output support}{d5_066}
{\Large $d=5$: basis element 66}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_066.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{19}$, \quad $\lambda=e^{i\frac{7\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_066.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 67: Additional output support}{d5_067}
{\Large $d=5$: basis element 67}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_067.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{21}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_067.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 68: Additional output support}{d5_068}
{\Large $d=5$: basis element 68}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_068.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{23}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_068.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 69: Additional output support}{d5_069}
{\Large $d=5$: basis element 69}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_069.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{25}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_069.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 70: Additional output support}{d5_070}
{\Large $d=5$: basis element 70}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_070.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{27}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_070.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 71: Additional output support}{d5_071}
{\Large $d=5$: basis element 71}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_071.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{29}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_071.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 72: Additional output support}{d5_072}
{\Large $d=5$: basis element 72}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_072.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{32}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_072.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 73: Additional output support}{d5_073}
{\Large $d=5$: basis element 73}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_073.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{34}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_073.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 74: Additional output support}{d5_074}
{\Large $d=5$: basis element 74}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_074.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{36}$, \quad $\lambda=e^{i\frac{7\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_074.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 75: Additional output support}{d5_075}
{\Large $d=5$: basis element 75}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_075.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{38}$, \quad $\lambda=e^{i\frac{\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=-\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_075.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 76: Additional output support}{d5_076}
{\Large $d=5$: basis element 76}\par
Additional output support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_076.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=X_{40}$, \quad $\lambda=e^{i\frac{7\pi}{4}}$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\frac{\pi}{2}$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_076.tikz}}}
\newpage
\pdfbookmark[1]{d=5: No boundary support}{group-5-internal}
\pdfbookmark[2]{d=5, element 77: No boundary support}{d5_077}
{\Large $d=5$: basis element 77}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_077.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_077.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 78: No boundary support}{d5_078}
{\Large $d=5$: basis element 78}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_078.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_078.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 79: No boundary support}{d5_079}
{\Large $d=5$: basis element 79}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_079.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_079.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 80: No boundary support}{d5_080}
{\Large $d=5$: basis element 80}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_080.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_080.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 81: No boundary support}{d5_081}
{\Large $d=5$: basis element 81}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_081.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_081.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 82: No boundary support}{d5_082}
{\Large $d=5$: basis element 82}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_082.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_082.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 83: No boundary support}{d5_083}
{\Large $d=5$: basis element 83}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_083.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_083.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 84: No boundary support}{d5_084}
{\Large $d=5$: basis element 84}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_084.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_084.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 85: No boundary support}{d5_085}
{\Large $d=5$: basis element 85}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_085.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_085.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 86: No boundary support}{d5_086}
{\Large $d=5$: basis element 86}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_086.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_086.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 87: No boundary support}{d5_087}
{\Large $d=5$: basis element 87}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_087.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_087.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 88: No boundary support}{d5_088}
{\Large $d=5$: basis element 88}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_088.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_088.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 89: No boundary support}{d5_089}
{\Large $d=5$: basis element 89}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_089.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_089.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 90: No boundary support}{d5_090}
{\Large $d=5$: basis element 90}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_090.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_090.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 91: No boundary support}{d5_091}
{\Large $d=5$: basis element 91}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_091.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_091.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 92: No boundary support}{d5_092}
{\Large $d=5$: basis element 92}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_092.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_092.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 93: No boundary support}{d5_093}
{\Large $d=5$: basis element 93}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_093.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_093.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 94: No boundary support}{d5_094}
{\Large $d=5$: basis element 94}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_094.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_094.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 95: No boundary support}{d5_095}
{\Large $d=5$: basis element 95}\par
No boundary support. Pauli web: no defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_095.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\vfill
{\footnotesize\texttt{\detokenize{d5_095.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 96: No boundary support}{d5_096}
{\Large $d=5$: basis element 96}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_096.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_096.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 97: No boundary support}{d5_097}
{\Large $d=5$: basis element 97}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_097.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_097.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 98: No boundary support}{d5_098}
{\Large $d=5$: basis element 98}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_098.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_098.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 99: No boundary support}{d5_099}
{\Large $d=5$: basis element 99}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_099.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_099.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 100: No boundary support}{d5_100}
{\Large $d=5$: basis element 100}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_100.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_100.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 101: No boundary support}{d5_101}
{\Large $d=5$: basis element 101}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_101.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_101.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 102: No boundary support}{d5_102}
{\Large $d=5$: basis element 102}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_102.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_102.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 103: No boundary support}{d5_103}
{\Large $d=5$: basis element 103}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_103.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_103.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 104: No boundary support}{d5_104}
{\Large $d=5$: basis element 104}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_104.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_104.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 105: No boundary support}{d5_105}
{\Large $d=5$: basis element 105}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_105.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_105.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 106: No boundary support}{d5_106}
{\Large $d=5$: basis element 106}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_106.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_106.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 107: No boundary support}{d5_107}
{\Large $d=5$: basis element 107}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_107.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_107.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 108: No boundary support}{d5_108}
{\Large $d=5$: basis element 108}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_108.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_108.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 109: No boundary support}{d5_109}
{\Large $d=5$: basis element 109}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_109.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_109.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 110: No boundary support}{d5_110}
{\Large $d=5$: basis element 110}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_110.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_110.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 111: No boundary support}{d5_111}
{\Large $d=5$: basis element 111}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_111.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_111.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 112: No boundary support}{d5_112}
{\Large $d=5$: basis element 112}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_112.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_112.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 113: No boundary support}{d5_113}
{\Large $d=5$: basis element 113}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_113.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_113.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 114: No boundary support}{d5_114}
{\Large $d=5$: basis element 114}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_114.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_114.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 115: No boundary support}{d5_115}
{\Large $d=5$: basis element 115}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_115.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_115.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 116: No boundary support}{d5_116}
{\Large $d=5$: basis element 116}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_116.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_116.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 117: No boundary support}{d5_117}
{\Large $d=5$: basis element 117}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_117.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_117.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 118: No boundary support}{d5_118}
{\Large $d=5$: basis element 118}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_118.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_118.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 119: No boundary support}{d5_119}
{\Large $d=5$: basis element 119}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_119.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_119.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 120: No boundary support}{d5_120}
{\Large $d=5$: basis element 120}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_120.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_120.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 121: No boundary support}{d5_121}
{\Large $d=5$: basis element 121}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_121.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_121.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 122: No boundary support}{d5_122}
{\Large $d=5$: basis element 122}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_122.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_122.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 123: No boundary support}{d5_123}
{\Large $d=5$: basis element 123}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_123.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_123.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 124: No boundary support}{d5_124}
{\Large $d=5$: basis element 124}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_124.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_124.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 125: No boundary support}{d5_125}
{\Large $d=5$: basis element 125}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_125.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_125.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 126: No boundary support}{d5_126}
{\Large $d=5$: basis element 126}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_126.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_126.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 127: No boundary support}{d5_127}
{\Large $d=5$: basis element 127}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_127.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_127.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 128: No boundary support}{d5_128}
{\Large $d=5$: basis element 128}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_128.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_128.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 129: No boundary support}{d5_129}
{\Large $d=5$: basis element 129}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_129.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_129.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 130: No boundary support}{d5_130}
{\Large $d=5$: basis element 130}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_130.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_130.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 131: No boundary support}{d5_131}
{\Large $d=5$: basis element 131}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_131.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_131.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 132: No boundary support}{d5_132}
{\Large $d=5$: basis element 132}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_132.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_132.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 133: No boundary support}{d5_133}
{\Large $d=5$: basis element 133}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_133.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_133.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 134: No boundary support}{d5_134}
{\Large $d=5$: basis element 134}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_134.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_134.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 135: No boundary support}{d5_135}
{\Large $d=5$: basis element 135}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_135.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_135.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 136: No boundary support}{d5_136}
{\Large $d=5$: basis element 136}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_136.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_136.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 137: No boundary support}{d5_137}
{\Large $d=5$: basis element 137}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_137.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_137.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 138: No boundary support}{d5_138}
{\Large $d=5$: basis element 138}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_138.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_138.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 139: No boundary support}{d5_139}
{\Large $d=5$: basis element 139}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_139.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_139.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 140: No boundary support}{d5_140}
{\Large $d=5$: basis element 140}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_140.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_140.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 141: No boundary support}{d5_141}
{\Large $d=5$: basis element 141}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_141.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_141.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 142: No boundary support}{d5_142}
{\Large $d=5$: basis element 142}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_142.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_142.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 143: No boundary support}{d5_143}
{\Large $d=5$: basis element 143}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_143.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_143.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 144: No boundary support}{d5_144}
{\Large $d=5$: basis element 144}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_144.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_144.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 145: No boundary support}{d5_145}
{\Large $d=5$: basis element 145}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_145.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_145.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 146: No boundary support}{d5_146}
{\Large $d=5$: basis element 146}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_146.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_146.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 147: No boundary support}{d5_147}
{\Large $d=5$: basis element 147}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_147.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_147.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 148: No boundary support}{d5_148}
{\Large $d=5$: basis element 148}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_148.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_148.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 149: No boundary support}{d5_149}
{\Large $d=5$: basis element 149}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_149.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_149.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 150: No boundary support}{d5_150}
{\Large $d=5$: basis element 150}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_150.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_150.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 151: No boundary support}{d5_151}
{\Large $d=5$: basis element 151}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_151.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_151.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 152: No boundary support}{d5_152}
{\Large $d=5$: basis element 152}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_152.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_152.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 153: No boundary support}{d5_153}
{\Large $d=5$: basis element 153}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_153.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_153.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 154: No boundary support}{d5_154}
{\Large $d=5$: basis element 154}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_154.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_154.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 155: No boundary support}{d5_155}
{\Large $d=5$: basis element 155}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_155.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_155.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 156: No boundary support}{d5_156}
{\Large $d=5$: basis element 156}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_156.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_156.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 157: No boundary support}{d5_157}
{\Large $d=5$: basis element 157}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_157.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_157.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 158: No boundary support}{d5_158}
{\Large $d=5$: basis element 158}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_158.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_158.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 159: No boundary support}{d5_159}
{\Large $d=5$: basis element 159}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_159.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_159.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 160: No boundary support}{d5_160}
{\Large $d=5$: basis element 160}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_160.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_160.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 161: No boundary support}{d5_161}
{\Large $d=5$: basis element 161}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_161.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_161.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 162: No boundary support}{d5_162}
{\Large $d=5$: basis element 162}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_162.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_162.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 163: No boundary support}{d5_163}
{\Large $d=5$: basis element 163}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_163.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_163.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 164: No boundary support}{d5_164}
{\Large $d=5$: basis element 164}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_164.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_164.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 165: No boundary support}{d5_165}
{\Large $d=5$: basis element 165}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_165.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_165.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 166: No boundary support}{d5_166}
{\Large $d=5$: basis element 166}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_166.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_166.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 167: No boundary support}{d5_167}
{\Large $d=5$: basis element 167}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_167.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_167.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 168: No boundary support}{d5_168}
{\Large $d=5$: basis element 168}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_168.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_168.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 169: No boundary support}{d5_169}
{\Large $d=5$: basis element 169}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_169.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_169.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 170: No boundary support}{d5_170}
{\Large $d=5$: basis element 170}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_170.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_170.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 171: No boundary support}{d5_171}
{\Large $d=5$: basis element 171}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_171.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_171.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 172: No boundary support}{d5_172}
{\Large $d=5$: basis element 172}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_172.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_172.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 173: No boundary support}{d5_173}
{\Large $d=5$: basis element 173}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_173.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_173.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 174: No boundary support}{d5_174}
{\Large $d=5$: basis element 174}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_174.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_174.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 175: No boundary support}{d5_175}
{\Large $d=5$: basis element 175}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_175.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_175.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 176: No boundary support}{d5_176}
{\Large $d=5$: basis element 176}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_176.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_176.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 177: No boundary support}{d5_177}
{\Large $d=5$: basis element 177}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_177.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_177.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 178: No boundary support}{d5_178}
{\Large $d=5$: basis element 178}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_178.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_178.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 179: No boundary support}{d5_179}
{\Large $d=5$: basis element 179}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_179.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_179.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 180: No boundary support}{d5_180}
{\Large $d=5$: basis element 180}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_180.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_180.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 181: No boundary support}{d5_181}
{\Large $d=5$: basis element 181}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_181.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_181.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 182: No boundary support}{d5_182}
{\Large $d=5$: basis element 182}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_182.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_182.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 183: No boundary support}{d5_183}
{\Large $d=5$: basis element 183}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_183.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_183.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 184: No boundary support}{d5_184}
{\Large $d=5$: basis element 184}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_184.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_184.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 185: No boundary support}{d5_185}
{\Large $d=5$: basis element 185}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_185.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_185.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 186: No boundary support}{d5_186}
{\Large $d=5$: basis element 186}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_186.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_186.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 187: No boundary support}{d5_187}
{\Large $d=5$: basis element 187}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_187.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_187.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 188: No boundary support}{d5_188}
{\Large $d=5$: basis element 188}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_188.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_188.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 189: No boundary support}{d5_189}
{\Large $d=5$: basis element 189}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_189.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_189.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 190: No boundary support}{d5_190}
{\Large $d=5$: basis element 190}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_190.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_190.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 191: No boundary support}{d5_191}
{\Large $d=5$: basis element 191}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_191.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_191.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 192: No boundary support}{d5_192}
{\Large $d=5$: basis element 192}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_192.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_192.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 193: No boundary support}{d5_193}
{\Large $d=5$: basis element 193}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_193.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_193.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 194: No boundary support}{d5_194}
{\Large $d=5$: basis element 194}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_194.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_194.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 195: No boundary support}{d5_195}
{\Large $d=5$: basis element 195}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_195.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_195.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 196: No boundary support}{d5_196}
{\Large $d=5$: basis element 196}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_196.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_196.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 197: No boundary support}{d5_197}
{\Large $d=5$: basis element 197}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_197.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_197.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 198: No boundary support}{d5_198}
{\Large $d=5$: basis element 198}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_198.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_198.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 199: No boundary support}{d5_199}
{\Large $d=5$: basis element 199}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_199.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_199.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 200: No boundary support}{d5_200}
{\Large $d=5$: basis element 200}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_200.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_200.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 201: No boundary support}{d5_201}
{\Large $d=5$: basis element 201}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_201.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_201.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 202: No boundary support}{d5_202}
{\Large $d=5$: basis element 202}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_202.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_202.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 203: No boundary support}{d5_203}
{\Large $d=5$: basis element 203}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_203.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_203.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 204: No boundary support}{d5_204}
{\Large $d=5$: basis element 204}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_204.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_204.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 205: No boundary support}{d5_205}
{\Large $d=5$: basis element 205}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_205.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_205.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 206: No boundary support}{d5_206}
{\Large $d=5$: basis element 206}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_206.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_206.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 207: No boundary support}{d5_207}
{\Large $d=5$: basis element 207}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_207.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_207.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 208: No boundary support}{d5_208}
{\Large $d=5$: basis element 208}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_208.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_208.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 209: No boundary support}{d5_209}
{\Large $d=5$: basis element 209}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_209.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_209.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 210: No boundary support}{d5_210}
{\Large $d=5$: basis element 210}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_210.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_210.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 211: No boundary support}{d5_211}
{\Large $d=5$: basis element 211}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_211.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_211.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 212: No boundary support}{d5_212}
{\Large $d=5$: basis element 212}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_212.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_212.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 213: No boundary support}{d5_213}
{\Large $d=5$: basis element 213}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_213.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_213.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 214: No boundary support}{d5_214}
{\Large $d=5$: basis element 214}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_214.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_214.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 215: No boundary support}{d5_215}
{\Large $d=5$: basis element 215}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_215.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_215.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 216: No boundary support}{d5_216}
{\Large $d=5$: basis element 216}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_216.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_216.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 217: No boundary support}{d5_217}
{\Large $d=5$: basis element 217}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_217.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_217.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 218: No boundary support}{d5_218}
{\Large $d=5$: basis element 218}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_218.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_218.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 219: No boundary support}{d5_219}
{\Large $d=5$: basis element 219}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_219.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_219.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 220: No boundary support}{d5_220}
{\Large $d=5$: basis element 220}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_220.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_220.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 221: No boundary support}{d5_221}
{\Large $d=5$: basis element 221}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_221.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_221.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 222: No boundary support}{d5_222}
{\Large $d=5$: basis element 222}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_222.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_222.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 223: No boundary support}{d5_223}
{\Large $d=5$: basis element 223}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_223.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_223.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 224: No boundary support}{d5_224}
{\Large $d=5$: basis element 224}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_224.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_224.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 225: No boundary support}{d5_225}
{\Large $d=5$: basis element 225}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_225.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_225.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 226: No boundary support}{d5_226}
{\Large $d=5$: basis element 226}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_226.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_226.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 227: No boundary support}{d5_227}
{\Large $d=5$: basis element 227}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_227.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_227.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 228: No boundary support}{d5_228}
{\Large $d=5$: basis element 228}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_228.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_228.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 229: No boundary support}{d5_229}
{\Large $d=5$: basis element 229}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_229.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_229.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 230: No boundary support}{d5_230}
{\Large $d=5$: basis element 230}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_230.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_230.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 231: No boundary support}{d5_231}
{\Large $d=5$: basis element 231}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_231.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_231.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 232: No boundary support}{d5_232}
{\Large $d=5$: basis element 232}\par
No boundary support. 3 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_232.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_232.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 233: No boundary support}{d5_233}
{\Large $d=5$: basis element 233}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_233.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_233.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 234: No boundary support}{d5_234}
{\Large $d=5$: basis element 234}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_234.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_234.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 235: No boundary support}{d5_235}
{\Large $d=5$: basis element 235}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_235.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_235.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 236: No boundary support}{d5_236}
{\Large $d=5$: basis element 236}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_236.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_236.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 237: No boundary support}{d5_237}
{\Large $d=5$: basis element 237}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_237.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_237.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 238: No boundary support}{d5_238}
{\Large $d=5$: basis element 238}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_238.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_238.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 239: No boundary support}{d5_239}
{\Large $d=5$: basis element 239}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_239.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_239.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 240: No boundary support}{d5_240}
{\Large $d=5$: basis element 240}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_240.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_240.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 241: No boundary support}{d5_241}
{\Large $d=5$: basis element 241}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_241.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_241.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 242: No boundary support}{d5_242}
{\Large $d=5$: basis element 242}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_242.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_242.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 243: No boundary support}{d5_243}
{\Large $d=5$: basis element 243}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_243.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_243.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 244: No boundary support}{d5_244}
{\Large $d=5$: basis element 244}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_244.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_244.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 245: No boundary support}{d5_245}
{\Large $d=5$: basis element 245}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_245.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_245.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 246: No boundary support}{d5_246}
{\Large $d=5$: basis element 246}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_246.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_246.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 247: No boundary support}{d5_247}
{\Large $d=5$: basis element 247}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_247.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_247.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 248: No boundary support}{d5_248}
{\Large $d=5$: basis element 248}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_248.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_248.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 249: No boundary support}{d5_249}
{\Large $d=5$: basis element 249}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_249.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_249.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 250: No boundary support}{d5_250}
{\Large $d=5$: basis element 250}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_250.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_250.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 251: No boundary support}{d5_251}
{\Large $d=5$: basis element 251}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_251.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_251.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 252: No boundary support}{d5_252}
{\Large $d=5$: basis element 252}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_252.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_252.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 253: No boundary support}{d5_253}
{\Large $d=5$: basis element 253}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_253.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_253.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 254: No boundary support}{d5_254}
{\Large $d=5$: basis element 254}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_254.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_254.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 255: No boundary support}{d5_255}
{\Large $d=5$: basis element 255}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_255.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_255.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 256: No boundary support}{d5_256}
{\Large $d=5$: basis element 256}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_256.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_256.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 257: No boundary support}{d5_257}
{\Large $d=5$: basis element 257}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_257.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_257.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 258: No boundary support}{d5_258}
{\Large $d=5$: basis element 258}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_258.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_258.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 259: No boundary support}{d5_259}
{\Large $d=5$: basis element 259}\par
No boundary support. 2 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_259.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_259.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 260: No boundary support}{d5_260}
{\Large $d=5$: basis element 260}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_260.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_260.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 261: No boundary support}{d5_261}
{\Large $d=5$: basis element 261}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_261.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_261.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 262: No boundary support}{d5_262}
{\Large $d=5$: basis element 262}\par
No boundary support. 4 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_262.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_262.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 263: No boundary support}{d5_263}
{\Large $d=5$: basis element 263}\par
No boundary support. 6 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_263.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$;\quad $\delta_{5}=\pi$;\quad $\delta_{6}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_263.tikz}}}
\newpage
\pdfbookmark[2]{d=5, element 264: No boundary support}{d5_264}
{\Large $d=5$: basis element 264}\par
No boundary support. 6 phase defects.
\begin{center}
\semiwebinput{semiwebs/diagrams/d5_264.tikz}
\end{center}
\vspace{-1mm}
$P_{\rm in}=I$, \quad $P_{\rm out}=I$, \quad $\lambda=1$, \qquad $K P_{\rm in}=\lambda P_{\rm out}K_{\boldsymbol\delta}$.
\par\smallskip\begin{minipage}{.98\linewidth}\small Phase changes: $\delta_{1}=\pi$;\quad $\delta_{2}=\pi$;\quad $\delta_{3}=\pi$;\quad $\delta_{4}=\pi$;\quad $\delta_{5}=\pi$;\quad $\delta_{6}=\pi$.\end{minipage}
\vfill
{\footnotesize\texttt{\detokenize{d5_264.tikz}}}
\newpage

